The Forward-In-Time-Only Assumption in SmartNIC Resource Management: A Critique of Wave and the Case for Bilateral Interaction

The datacenter industry is converging on SmartNIC-based resource management. Wave (Humphries et al., ASPLOS '25) demonstrates the practical feasibility of offloading kernel thread scheduling, memory management, and RPC stacks to the ARM cores of Intel's Mount Evans Infrastructure Processing Unit (IPU). The engineering is careful and the results are honest: without Wave's PCIe latency mitigations, offloaded workloads degrade by 350%. We argue that this 350% degradation is not an engineering problem to be optimized away but a diagnostic symptom of a deeper architectural issue: Wave's communication model is Forward-In-Time-Only (FITO). Every interaction between host and SmartNIC is a unidirectional message -- event forward, decision back -- creating a temporal vulnerability window in which decisions can become stale before they are enforced. Wave's entire optimization stack (write-combining page table entries, prestaging, prefetching, atomic transaction abort) exists to hide or tolerate this window. We apply the FITO diagnostic to Wave's architecture systematically, identify the category mistake it inherits from Lamport's happened-before and Shannon's channel model, and show how Open Atomic Ethernet's bilateral swap primitive -- implemented on the same Intel IPU hardware -- dissolves the latency, atomicity, and timeout problems without engineering around them. The SmartNIC is the right location for resource management; what is missing is the right communication primitive at that location.

==> dae-handout-commands.tex <==
% --- dae_commands.tex ---

% --- FAQ/Answer macros ---
\newcommand{\question}[1]{%
  \stepcounter{qctr}%
  \vspace{5pt}
  \noindent
  \rule{0.5\columnwidth}{0.5pt}\\
  \noindent
  \phantomsection
  \textbf{[Q\decimal{qctr}]}~%
  \def\a##1\par{##1}{#1}%
  \addcontentsline{loq}{section}{Q\protect\numberline{\theqctr}{{#1}}}
}

\newcommand{\answer}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}]}
}

\newcommand{\statement}{%
  \vspace{5pt}
  \noindent
  \textbf{[S\decimal{qctr}] Statement: }
}

\newcommand{\insight}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}} Insight: ]
}

\newcommand{\sublistofquestions}{%
  \onlyinsubfile{\vspace{0pt} \large \listofquestions \normalsize \medskip}
}

% --- Subfiles helpers ---
\newcommand{\onlyinsubfile}[1]{#1}
\newcommand{\notinsubfile}[1]{}

% --- Insert Hyperlink (file) ---
\newcommand{\ihl}[2]{%
  \vspace{6pt} \noindent [\hyperlink{./Exhibits/#1.pdf.1}{#1}]{ #2}
}

% --- Insert Menu Item (file/comment) ---
\newcommand{\imi}[2]{%
  \vspace{10pt}
  \noindent
  \textbf{\href{run:FAQ-#1.pdf}{#1}}\\{#2}
}

% --- Strikeout Displaystyle ---
\newcommand{\displayst}[1]{\textrm{\st{$\displaystyle#1$}}}

% --- Custom Horizontal Rule ---
\newcommand{\srule}{%
  \vspace{2pt}
  \noindent\rule{\textwidth}{0.8pt}
}

% --- Leibniz Bridge sibling document references ─────────────────
% \daeref{label}{filename}{description}
%   Links to a sibling document in the same project folder.
%   Rendered in linkred. Margin note shows label + description.
%   Auto-detects format from extension and annotates [PDF] or [HTML].
%   Uses \href{run:filename} so macOS opens the right application.
%   In arXiv/HTML mode: becomes a footnote (no margin note).
%
% Usage:
%   \daeref{DAE-TR-0007}{DAE-TR-0007.pdf}{The Category Mistake}
%   \daeref{CAP Paper}{oae-cap-tufte.html}{HTML with responsive sidenotes}
%
\makeatletter
\newcommand{\dae@detectformat}[1]{%
  \dae@checkhtml#1.html\@nil
}
\def\dae@checkhtml#1.html#2\@nil{%
  \def\dae@temp{#2}%
  \ifx\dae@temp\empty
    \def\dae@fmt{PDF}%  no .html found, assume PDF
  \else
    \def\dae@fmt{HTML}%
  \fi
}
\ifarxiv
  \newcommand{\daeref}[3]{%
    \dae@detectformat{#2}%
    \href{#2}{\textcolor{linkred}{#1}}%
    \footnote{\textcolor{linkred}{#1}\enspace[\dae@fmt]\enspace #3}%
  }
\else
  \newcommand{\daeref}[3]{%
    \dae@detectformat{#2}%
    \href{run:#2}{\textcolor{linkred}{#1}}%
    \marginnote{\scriptsize\textcolor{linkred}{#1}\enspace\textsc{[\dae@fmt]}:\enspace #3}%
  }
\fi
\makeatother

% --- Leibniz Bridge Margin TOC (standardized) ---
% Usage: place \daemargintoc after \maketitle / \placebadges on the first page.
% Requires: etoc, hyperref, linkgreen colour defined,
%           Bitstream Charter via mathdesign (provides bold small caps).
% Sections: bold small caps, green, with number.
% Subsections: regular small caps, green, indented.
% Section short titles MUST be in Title Case for the small-caps effect.
% In arXiv/HTML mode: suppressed (arXiv generates its own TOC sidebar).
\newcommand{\daemargintoc}{%
  \ifarxiv\else
  \marginnote{%
    \hypersetup{linkcolor=linkgreen}%
    \small
    \setcounter{tocdepth}{2}%
    \etocsetstyle{section}{}{\par\vspace{1em}\noindent\leftskip=0em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textbf{\textsc{\etocname}}}%
      \hfill\etocpage\par}{}{}%
    \etocsetstyle{subsection}{}{\par\vspace{0.5em}\noindent\leftskip=1.5em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textsc{\etocname}}%
      \hfill\etocpage\par}{}{}%
    \etocsettocstyle{}{}%
    \tableofcontents
  }%
  \fi
}

\NewDocumentCommand{\marginfig}{O{width=\linewidth} m o o o o}{%
  \begin{marginfigure}\IfValueT{#6}{[#6]}%
    \IfValueTF{#5}{#5}{\centering}%
    \includegraphics[#1]{#2}%
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{marginfigure}
}

\NewDocumentCommand{\fig}{O{width=\linewidth} m o o}{%
  \begin{figure}
    \centering
    \includegraphics[#1]{#2}% 
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{figure}
}


==> dae-handout-settings.tex <==
% Document class

% Core packages
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}
\usepackage{xparse}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{lipsum}
\usepackage{epigraph}
\usepackage{framed}
\usepackage{todonotes}
\usepackage[most]{tcolorbox}

% Specialized
\usepackage{tikz}
% \usepackage{bytefield}  % Not needed for this paper
\usepackage{eso-pic}

% Graphics path (Leibniz Bridge convention):
%   ./figures/    — local working copies (populated by pull-figures.sh)
%   ../Figures/   — shared parent folder
%   ../../Figures/ — grandparent
%   FIGURES/      — absolute iCloud master (last resort)
\graphicspath{{./}{./figures/}{../Figures/}{../../Figures/}{./images/}{./graphics/}}

% ── Leibniz Bridge colour scheme ─────────────────────────────────
% Green: internal navigation (same document) — \ref, \cite, TOC
% Blue:  external web links — \url, \href to http(s)
% Red:   sibling documents (PDF, HTML in same project folder)
\definecolor{linkblue}{RGB}{30, 80, 180}
\definecolor{linkgreen}{RGB}{30, 120, 60}
\definecolor{linkred}{HTML}{AE0000}

% Hyperref
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  urlcolor=linkblue,          % \url and \href to web
  linkcolor=linkgreen,        % \ref, \eqref, \pageref, TOC
  citecolor=linkgreen,        % \cite (jumps to bib within this doc)
  filecolor=linkred,          % \href{run:...} local file links
}

% Font commands
\newcommand{\headerfont}{\fontfamily{phv}\selectfont}
\newcommand{\titlefont}{\headerfont\Huge\bfseries}
\newcommand{\authorfont}{\headerfont\large}
\newcommand{\datefont}{\headerfont\normalsize}

% Custom title page
\makeatletter
\renewcommand{\maketitle}{
  \newpage
  \thispagestyle{empty}
  \begin{fullwidth}
    \centering
    {\titlefont \@title \par}
    \vspace{1em}
    \ifx\@author\@empty\else
      {\authorfont \@author \par}
      \vspace{0.5em}
    \fi
    \ifx\@date\@empty\else
      {\datefont \@date \par}
    \fi
    \vspace{2em}
  \end{fullwidth}
}
\makeatother

% Custom abstract
\newenvironment{customabstract}{
  \begin{fullwidth}
  \begin{adjustwidth}{0.5in}{0.5in}
  \vspace{1em}
  \small
  \color{gray!30!black}
}{
  \vspace{1.5em}
  \end{adjustwidth}
  \end{fullwidth}
}



% Unicode fallback
\DeclareUnicodeCharacter{2E3B}{\textbar\textbar}

% Optional: comment out subfiles you're not using
%\includeonly{Protocol-Byte-Content}


==> fito-marginbox.tex <==
% ══════════════════════════════════════════════════════════════════
% FITO MARGIN BOX - Reusable component for Tufte documents
% ══════════════════════════════════════════════════════════════════
% Usage: \input{fito-marginbox}  in preamble
%        \fitobox               where you want the margin note
%        \fitoboxshort          for a condensed version
%
% Requires: xcolor, tikz (typically already loaded in tufte docs)
% ══════════════════════════════════════════════════════════════════

% ── Color definitions ───────────────────────────────────────────
\definecolor{fitered}{RGB}{180, 40, 40}          % Deep red for border/title
\definecolor{fitobg}{RGB}{255, 245, 245}         % Very light red background
\definecolor{fitotext}{RGB}{80, 20, 20}          % Dark red-brown for text

% ── TikZ settings for the box ───────────────────────────────────
\usetikzlibrary{calc}

% ── The FITO Box Command (full version) ─────────────────────────
\newcommand{\fitobox}{%
  \marginnote{%
    \begin{tikzpicture}
      \node[
        draw=fitered,
        line width=1.2pt,
        fill=fitobg,
        rounded corners=3pt,
        inner sep=6pt,
        text width=\marginparwidth-16pt,
        align=left
      ] {%
        {\bfseries\color{fitered}\footnotesize FITO}\\[3pt]
        {\scriptsize\color{fitotext}%
        \textbf{Forward-In-Time-Only}: the assumption that causation,
        ordering, and correctness flow unidirectionally through time.\\[4pt]
        \textit{Consequences:}\\[2pt]
        \hangindent=0.8em\hangafter=1
        • Corrupted data structures from race conditions\\[1pt]
        \hangindent=0.8em\hangafter=1
        • Database logs that cannot be reconciled\\[1pt]
        \hangindent=0.8em\hangafter=1
        • Coordination failures masked as ``network errors''\\[1pt]
        \hangindent=0.8em\hangafter=1
        • Impossibility theorems mistaken for physical laws%
        }%
      };
    \end{tikzpicture}%
  }%
}

% ── The FITO Box Command (short version) ────────────────────────
\newcommand{\fitoboxshort}{%
  \marginnote{%
    \begin{tikzpicture}
      \node[
        draw=fitered,
        line width=1.2pt,
        fill=fitobg,
        rounded corners=3pt,
        inner sep=5pt,
        text width=\marginparwidth-14pt,
        align=left
      ] {%
        {\bfseries\color{fitered}\footnotesize FITO}\\[2pt]
        {\scriptsize\color{fitotext}%
        \textbf{Forward-In-Time-Only}: causation flows one way through
        monotonic time.  Leads to corrupted state, unreconcilable logs,
        coordination failures.%
        }%
      };
    \end{tikzpicture}%
  }%
}

% ── Inline definition (for running text) ────────────────────────
\newcommand{\fitoinline}{%
  {\color{fitered}\textbf{FITO}} (Forward-In-Time-Only)%
}

